Queen: A quick, scalable, and comprehensive quantum circuit simulation for supercomputing

The state vector-based simulation offers a convenient approach to developing and validating quantum algorithms with noise-free results. However, limited by the absence of cache-aware implementations and unpolished circuit optimizations, the past simulators were severely constrained in performance, leading to stagnation in quantum computing. In this paper, we present an innovative quantum circuit simulation toolkit comprising gate optimization and simulation modules to address these performance challenges. For the performance, scalability, and comprehensive evaluation, we conduct a series of particular circuit benchmarks and strong scaling tests on a DGX-A100 workstation and achieve averaging 9 times speedup compared to state-of-the-art simulators, including QuEST, IBM-Aer, and NVIDIA-cuQuantum. Moreover, the critical performance metric FLOPS increases by up to a factor of 8-fold, and arithmetic intensity experiences a remarkable 96x enhancement. We believe the proposed toolkit paves the way for faster quantum circuit simulations, thereby facilitating the development of novel quantum algorithms.

==> contents/AD.tex <==
\section{Artifact Evaluation (AD)}
\subsection{Paper's Main Contributions}
\begin{description}
\item [$C_1$] This paper introduces an all-in-one optimization module designed to convert original quantum circuits into optimized versions that are more tailored for execution on classical computers.
\item [$C_2$] This paper presents the implementation and performance analysis of the all-in-cache simulation module with a high-speed simulation workflow.
\item[$C_3$] This paper conducts a comparative analysis of simulation performance utilizing qubit, gate, and circuit benchmarks on multi-GPUs against state-of-the-art simulators.
\end{description}

\subsection{Computational Artifacts}
To safeguard against unauthorized use, please email to the authors.

\begin{center}
\begin{tabular}{rll}
\toprule
Artifact ID  &  Contributions &  Related \\
             &  Supported     &  Paper Elements \\
\midrule
$A_1$ & $C_1$ & Figure 5 \\
\midrule
$A_2$ & $C_2$, $C_3$ & Figure 8 \\
& & Figure 9 \\
& & Figure 10 \\
& & Figure 11 \\
& & Figure 12 \\
%\midrule
\bottomrule
\end{tabular}
\end{center}

\begin{center}
    \textbf{\noindent{Artifact Identification}}
\end{center}

\subsection{Computational Artifact A1}
\noindent\textit{Relation To Contributions}

This artifact $A_1$ is an implementation of $C_1$, which is an optimization tool for doing the qubit reordering and gate fusion within the quantum circuits.

\noindent\textit{Expected Results}

This artifact aims to transform any circuits (e.g., QFT, QAOA, or BV) into the optimized circuit file, which includes gate blocks, in-memory swapping (SQS), and cross-device swapping (CSQS).
Specifically, the input format for the circuit is structured as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{[Gate type] \textcolor{red}{[Target qubits]} [ID] [Remain info]}
\end{tcolorbox}
\end{center}

Given an example circuit represented in Figure 5 (a), along with our specified input format, the optimization module is capable of producing the optimized circuit as output.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{H \textcolor{red}{0} 0}
\\\textbf{ H \textcolor{red}{1} 1}
\\\textbf{ RZZ \textcolor{red}{2 4} 2}
\\\textbf{ RZZ \textcolor{red}{5 7} 3}
\\\textbf{ H \textcolor{red}{8} 4}
\\\textbf{ H \textcolor{red}{9} 5}
\\\textbf{ H \textcolor{red}{3} 6}
\\\textbf{ H \textcolor{red}{6} 7}
\\\textbf{ RZZ \textcolor{red}{0 2} 8}
\\\textbf{ RZZ \textcolor{red}{4 7} 9}
\\\textbf{ H \textcolor{red}{9} 10}
\\\textbf{ RZZ \textcolor{red}{1 8} 11}
\\\textbf{ RZZ \textcolor{red}{3 6} 12}
\\\textbf{ H \textcolor{red}{5} 13}
\end{tcolorbox}
\end{center}

The output resulting from the qubit reordering optimization should match Figure 5(b) as follows.
The target qubit for each original gate operation should not exceed the chunk size of 4, which is also marked in red.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{3} \textcolor{ForestGreen}{\# Gate Block Size}
\\\textbf{H \textcolor{red}{0} 0}
\\\textbf{H \textcolor{red}{1} 1}
\\\textbf{H \textcolor{red}{3} 6}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 5 7} \textcolor{ForestGreen}{\# In-memory swapping}
\\\textbf{4}
\\\textbf{RZZ \textcolor{red}{0 2} 2}
\\\textbf{RZZ \textcolor{red}{1 3} 3}
\\\textbf{RZZ \textcolor{red}{0 3} 9}
\\\textbf{H \textcolor{red}{1} 13}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 6 7}
\\\textbf{3}
\\\textbf{H \textcolor{red}{1} 7}
\\\textbf{RZZ \textcolor{red}{1 3} 12}
\\\textbf{RZZ \textcolor{red}{0 2} 8}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{CSQS 2 6 7 8 9} \textcolor{ForestGreen}{\# Cross-device swapping}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{SQS 1 3 5}
\\\textbf{4}
\\\textbf{H \textcolor{red}{2} 5}
\\\textbf{H \textcolor{red}{2} 10}
\\\textbf{H \textcolor{red}{0} 4}
\\\textbf{RZZ \textcolor{red}{0 3} 11}
\end{tcolorbox}
\end{center}

After applying all features in this module, the result should match Figure 5(c). The diagonal gates, such as RZZ, within each gate block, will be merged without altering correctness.
To avoid excessive elaboration, detailed results are not provided.
Please verify this matter effortlessly through the scripts we provided.

To verify the optimized circuit executes in the correct sequence and with proper dependencies
on target qubits, one can utilize our validation script as follows.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!75!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the validation directory}
\\
\textbf{\$ cd ./tests}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# run the validation script}
\\
\textbf{\$ ./validate\_circuit\_order.sh}
\end{tcolorbox}
\end{center}


If all optimized circuits have the correct sequence, the message "Passed all circuit order validations" will be output to the terminal. Otherwise, a mismatch error will be invoked.

\noindent\textit{Expected Reproduction Time (in Minutes)}
% \artexpl{
% Estimate the time required to reproduce the artifact, providing separate estimates for the individual steps: Artifact Setup, Artifact Execution, and Artifact Analysis.
% }

The expected results of this module are listed as follows.
\begin{easylist}
& The required time for Artifact Setup is negligible if our provided raw circuit file is adopted. Otherwise, installing the Python package of the open-source project may take 5-10 minutes.
& For Artifact Execution, each optimized circuit of our benchmark is consistently generated within 0.5 seconds.
& For Artifact Analysis, the optimized circuit does not represent the actual simulation efficiency, so we refrain from discussing it for now.
\end{easylist}

\noindent\textit{Artifact Setup (incl. Inputs)}

\textit{Hardware:} No specific Hardware is required to execute the experiments.

\textit{Operating System:} We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. However, no specific operating system is required to execute the experiments.

\textit{Software:} No specific software is required to execute the experiments.
However, for the convenience of downloading the open-source circuit generator and facilitating subsequent simulation stages, we still recommend installing all necessary environments at this stage.

\begin{easylist}
& In order to generate highly reproducible circuits in an open-source manner and facilitate direct comparisons with various works in one single execution environment, Python 3.10.12 should be used along with the following package dependencies. (i.e., using different configurations does not ensure running the experiments for all related works in one single environment):
    && attrs==20.3.0
    && cachetools==5.3.3
    && certifi==2021.5.30
    && charset-normalizer==3.3.2
    && cirq==0.13.1
    && cirq-aqt==0.13.1
    && cirq-core==0.13.1
    && cirq-google==0.13.1
    && cirq-ionq==0.13.1
    && cirq-pasqal==0.13.1
    && cirq-rigetti==0.13.1
    && cirq-web==0.13.1
    && contourpy==1.2.0
    && cuquantum-cu12==23.10.0
    && custatevec-cu12==1.5.0
    && cutensor-cu12==1.7.0
    && cutensornet-cu12==2.3.0
    && cycler==0.12.1
    && decorator==5.1.1
    && dill==0.3.8
    && duet==0.2.9
    && fonttools==4.49.0
    && google-api-core==1.34.1
    && google-auth==2.28.2
    && googleapis-common-protos==1.63.0
    && grpcio==1.62.1
    && grpcio-status==1.48.2
    && h11==0.9.0
    && httpcore==0.11.1
    && httpx==0.15.5
    && idna==2.10
    && iso8601==0.1.16
    && kiwisolver==1.4.5
    && lark==0.11.3
    && matplotlib==3.8.3
    && mpmath==1.3.0
    && msgpack==1.0.8
    && networkx==2.8.8
    && numpy==1.26.4
    && nvidia-cublas-cu12==12.3.4.1
    && nvidia-cuda-runtime-cu12==12.3.101
    && nvidia-cusolver-cu12==11.5.4.101
    && nvidia-cusparse-cu12==12.2.0.103
    && nvidia-nvjitlink-cu12==12.3.101
    && packaging==24.0
    && pandas==2.2.1
    && pbr==6.0.0
    && pillow==10.2.0
    && ply==3.11
    && protobuf==3.20.3
    && psutil==5.9.8
    && py==1.11.0
    && pyasn1==0.5.1
    && pyasn1-modules==0.3.0
    && pydantic==1.8.2
    && PyJWT==1.7.1
    && pyparsing==3.1.2
    && pyquil==3.0.1
    && python-dateutil==2.8.2
    && python-rapidjson==1.16
    && pytz==2024.1
    && pyzmq==25.1.2
    && qcs-api-client==0.8.0
    && qiskit==0.46.0
    && qiskit-aer-gpu==0.13.3
    && qiskit-terra==0.46.0
    && requests==2.31.0
    && retry==0.9.2
    && retrying==1.3.4
    && rfc3339==6.2
    && rfc3986==1.5.0
    && rpcq==3.11.0
    && rsa==4.9
    && ruamel.yaml==0.18.6
    && ruamel.yaml.clib==0.2.8
    && rustworkx==0.14.2
    && scipy==1.12.0
    && six==1.16.0
    && sniffio==1.2.0
    && sortedcontainers==2.4.0
    && stevedore==5.2.0
    && symengine==0.11.0
    && sympy==1.12
    && toml==0.10.2
    && tqdm==4.66.2
    && typing\_extensions==4.10.0
    && tzdata==2024.1
    && urllib3==2.2.1
\end{easylist}

\textit{Datasets / Inputs:} To lessen the load on users for recompilation, the experimental inputs consist of a designated configuration file and a total of 17 distinct gates and circuits, accessible via the ./circuit directory.
Alternatively, one can also generate all the raw circuits with the following command.

\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# install required packages listed in the \emph{Software} section}
\\
\textbf{\$ pip3 install -r requirements.txt}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./optimizer}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# generate raw circuits (e.g., BV, QAOA, ..., etc) }
\\
\textbf{\$ ./gen\_raw\_circuits.sh}
\\
\end{tcolorbox}
\end{center}

\textit{Installation and Deployment:}
The version of the GNU g++ compiler used is 11.04.

\noindent\textit{Artifact Execution}
A workflow may consist of two tasks: $T_1$ and $T_2$.
Task $T_1$ compiles the C++ source code for the all-in-one module.
Task $T_2$ leverages the module to transform the raw circuits in all experiments into optimized circuits.
The dependency of tasks is $T_1 \rightarrow T_2$
Note that the raw circuits have already been obtained in the \emph{dataset/input} section.

\noindent\textit{Artifact Analysis (incl. Outputs)}
In terms of efficiency, the elapsed time for transforming any raw circuit is less than 1 second on a DGX-A100, thanks to the polynomial-time complexity of the implementation.

Moreover, this artifact demonstrates promising results in reducing the number of gate blocks.
For example, the 31-qubit QFT circuit with 496 gates is grouped into only 18 gate blocks.
Theoretically, memory access time could be reduced by a factor of 27 (496/18). However, in practice, this reduction is usually unattainable due to considerations involving compiler optimizations, making it more of a reference point.

The reductions in gate blocks result in fewer in-memory swaps and cross-device swaps compared to other works, thereby enhancing an 8-fold times speedup while running the circuit through our simulation module ($A_2$) on the DGX-A100, a significance that is elaborated upon in more depth in the AE.

\subsection{Computational Artifact A2}
\noindent\textit{Relation To Contributions}

This artifact $A_2$ is a comprehensive tool for quantum circuit simulation that orchestrates the complete implementation of $C_2$.
%Running this artifact with a performance profiler yields the results of $C_3$ on the given machines.
The integration of various benchmarks and other simulators can showcase the efficiency of $C_3$ (i.e., demonstrating higher efficiency compared to the other works).
Alongside the generated circuit via artifact $A_1$, this stage enables the presentation of a comprehensive performance report.

\noindent\textit{Expected Results}

The expected results of each benchmark on a DGX-A100 workstation are listed as follows.
These benchmarking results can dominate state vector-based simulation in various cases, as mentioned in 

\begin{easylist}
& QAOA Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& QFT Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& Qubit Benchmark: \\Our work should get an average performance improvement of 9.x compared to cuQuantum and Aer in various qubit scenarios.
& Strong Scaling Benchmark: \\This experiment demonstrates that our work has strong scaling capability, achieving an average performance improvement of 8.7x compared to cuQuantum and Aer in various device scenarios.
& Gate Benchmark: \\ To show the versatility of various gates, our work should get an average performance improvement of 8.7x compared to cuQuantum and Aer.
& Circuit Benchmark: \\To show the versatility of various circuits, our work should get an average performance improvement of 9.x compared to cuQuantum and Aer.
& Breakdown of 34-qubit Simulation Time: \\Gate operation should occupy the most time. This experiment can be used to analyze the whole simulation process for different circuits.
& Breakdown of 34-qubit Simulation Time w/o NVLink and shared memory: \\The cross-device swapping should occupy the most time. This experiment serves as a benchmark for comparison against NVLink and socket-based methodologies.
& Roofline Model of The 30-qubit H-gate Benchmark: \\Our work should be computation-bound, while QuEST should be memory-bound, highlighting the decisive difference that demonstrates us as the next-generation simulator.
\end{easylist}

\arttime

\begin{easylist}
& For Artifact Setup, the required time is negligible if our Dockerfile is adopted. 
Otherwise, installing the NVIDIA Driver, CUDA toolkit, and NCCL library may take up to 30 minutes, depending on network speed.

& For Artifact Execution, we provide the expected computational time of this artifact on a DGX-A100 as follows.
Notably, the proficiency with which information is gathered using a profiler varies depending on the familiarity with the operations.
    && QAOA Benchmark: 16 minutes
    && QFT Benchmark: 5 minutes
    && Qubit Benchmark: 4 minutes
    && Strong Scaling Benchmark: 3 minutes
    && Gate Benchmark: 15 minutes
    && Circuit Benchmark: 15 minutes
    && Breakdown of 34-qubit Simulation Time: 15 minutes
    && Breakdown of 34-qubit Simulation Time without NVLink: 150 minutes
    && Roofline Model: 3 minutes
& For Artifact Analysis, the required time is negligible when utilizing our provided script, which summarizes the results into a CSV and PDF file for each experiment.
%Otherwise, each experiment may take 5-10 minutes to discern the parameters and input for various simulators.
\end{easylist}

\artin

\artinpart{Hardware}

For the experiments, we use a DGX-A100 workstation comprising two AMD EPYC 7742 CPUs and eight NVIDIA A100 SXM GPUs interconnected via NVLink, boasting a bandwidth of 600GB/s.

\artinpart{Operating System}
We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. 
However, no specific operating system is required to execute the experiments.

\artinpart{Software}
We use NVCC ver. 12.3.107 and the NCCL library ver. 2.20.3.
To reproduce the related works, the Python environment matches that of artifact $A_1$. You also need cmake to build QuEST, the related work we compared our work against. The version of cmake we use is ver. 3.22.1.

\artinpart{Datasets / Inputs}
All circuit inputs can be obtained after completing the steps of artifact $A_1$.

\artinpart{Installation and Deployment}

For compilation, we use NVCC ver. 12.3.107 with the "-lnccl -arch=sm\_80 -O3 
-{}- jump-table-density=0 -maxrregcount=64" flags and the NCCL library ver. 2.20.3 for compiling the CUDA codes.

To compile the executable file, execute "make -j" in the terminal within the ./simulator directory of the workspace path, and no specific requirements for deploying our work.

To execute the experiments, ensure the configure and circuit files exist, then run it with the following suggested command.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./simulator/Quokka -i [configure file] -c [circuit file]}
\end{tcolorbox}
\end{center}

\artcomp

A workflow may consist of three tasks: $T_1$, and $T_2$.
The task $T_1$ generates specific configure files, quantum gates, and circuits as benchmarks with optimizations for the simulators\footnote{The task $T_1$ represents the entire process of artifact $A_1$. If already completed, please skip this step.
}.
These configurations and benchmarks are then used as input by computational task $T_2$.
The outputs can be directly displayed in the terminal.
The results can also be automatically summarized as a CSV and PDF file if one utilizes our provided scripts.
%With a comprehensive chart or additional plotting package in task $T_3$, exquisite performance reports can be presented.
The dependencies for reproducing our work are as follows: $T_1 \rightarrow T_2$.
The detailed step-by-step reproduction will be detailed in the Artifact Evaluation section.

The details of the experimental parameters are listed as follows.
\begin{easylist}
& In our simulator, specifying the size of the simulated qubits is achieved by switching the configuration file. This can be done by modifying the value of N in the .ini file.
& In our simulator, simulating different circuits only requires switching the .txt file without the need for recompilation.
Rest assured, our scripts, codes with comments, and README.md files offer abundant examples to aid in completing all experiments.
& The default number of qubits in the A100 scenario is set to 31 (this is the memory upper limit), but please adjust it according to your GPUs.
& There are 7 practical quantum circuits and 10 standard quantum gates used as benchmarks. 
You can still generate specific simulation circuit files according to your needs, but please refer to the advanced user manual to complete this task.
& Given that the circuits executed in benchmarks and simulated scenarios are both large-scale, it is recommended to run the simulations multiple times to remove noise, even though running once is usually sufficient to indicate the simulation time.
\end{easylist}



Overall, we utilize the better elapsed time to identify a more effective simulation result.
A brief analysis and interpretation of each benchmark are listed below.
\begin{easylist}
& QAOA Benchmark:
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QAOA circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& QFT Benchmark: 
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QFT circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& Qubit Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with qubits ranging from 24 to 31.
It demonstrates the performance of the simulator under varying memory consumption levels.
Our work gets the fastest results for all cases on an A100.
& Strong scaling Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with devices ranging from 1 to 8 exponentially.
It demonstrates the robust scalability of the simulator under varying GPU devices.
Our work gets the fastest results for all cases on a DGX-A100.
& Gate benchmark:
\\This benchmark evaluates the time per gate for different types of gates on a 31-qubit system.
It demonstrates the high performance of each implementation for all varying gates.
Our work gets the fastest results for all cases on an A100.
& Circuit benchmark:
\\This benchmark evaluates the time per gate for different types of practical circuits on a 31-qubit system.
It demonstrates the high performance of each implementation for varying circuits.
Our work gets the fastest results for all cases on an A100.
& Breakdown of 34-qubit simulation time:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models, with NVLink serving as the transfer medium for cross-device communication.
Observing the changes in elapsed time, it can be noted that introducing in-memory swapping and cross-device swapping is highly beneficial.
& Breakdown of 34-qubit simulation time without NVLink and shared memory:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models without relying on NVLink for cross-device communication. Observing the changes in elapsed time, it can be noted that utilizing NVLink for cross-device swapping is highly beneficial.
& Roofline model of the 30-qubit H-gate benchmark: \
\\This analysis is typically used to determine whether the application is computation-bound or memory-bound.
By utilizing the Nsight Compute profiler, it is evident that our simulator is computation-bound across different levels of GPU.
For other simulators (we take QuEST as an example), the performance is significantly limited by memory bandwidth.
\end{easylist}

==> contents/ralated_work.tex <==
\section{Related Work}
\label{sec:related_work}
%\fixme{cite some papers in this section}
% 1 State vector 的好處是什麼 vs other
% 這樣的模擬器是和平行話地運算，所以適合在超級電腦上模擬（開蹭
% 模擬快速尤其需要不同模擬層面跟店路層面做不同層面的分析與探討
\begin{comment}
\fixme{
Distributed state vector simulators have been developed to
simulate large-scale quantum circuits on multiple computing
nodes. They can utilize the computational power and memory
capacity of multiple nodes by distributing a state vectocross them. In this section, we introduce four state-of-theart distributed simulators: Intel-QS, QuEST, JUQCS-G, and
Qiskit Aer.
\end{comment}
%There are basically two kinds of methods for simulating quan- tum circuits. The first kind is called state-vector simulation or Schrödinger method [1, 2, 9, 16, 17, 24, 26, 28–30], which stores the full states of the qubits in memory and updates them with each quan- tum gate operation. Because all quantum states can be measured directly in the processing of the simulation, it is convenient for researchers to debug quantum programs and perform other opera- tions. Another kind of method is the tensor approach that performs the simulation by contracting a tensor network [3, 5, 6, 20, 23, 27]. Since its computing complexity is directly related to the entanglement generation of the underlying quantum circuit [13], it is not suitable for the complex quantum circuit (such as Sycamore) and unable to support quantum program debugging [19].

Quantum circuit simulation can be typically categorized into state vector-based and tensor network-based approaches.
While tensor networks are limited in terms of interpretability and scalability, state vector-based QCS is widely preferred for its superior ability to represent complex quantum circuits with high scalability accurately.
Additionally, state vector-based QCS is highly parallelizable, making it ideal for execution on supercomputers~\cite{QuEST, 45qubit, TaihuLight, qHiPSTER, cuQuantum, cache_blocking}.
To achieve effective QCS, it is essential to consider complementary optimization strategies for both the simulation and circuit analysis levels.

%The state vector-based quantum circuit simulator plays a crucial role in simulating the total quantum state of both noisy and noise-free quantum circuits. Due to the inherently parallel nature of statevector simulator calculations, it proves highly conducive to execution on supercomputers~\cite{QuEST}. However, achieving an effective QCS entails the formulation of complementary optimization strategies for both the simulation and circuit analysis levels.

% 
% 模擬層面是： 特性是和平行計算, 與分散式計算
\begin{comment}
\textbf{Full-state simulation.}
ptimizations in full-state simulation. To improve simula- tion performance, some full-state simulators apply vectorization[1, 9, 16], support GPU acceleration[1, 9, 28], and perform distributed processing[28]. Also, they apply many optimization techniques, such as cache blocking[41] gate scheduling, and gate fusion[1, 9]. Fatima et al.[22] propose a highly optimized simulation algorithm that uses the single-precision floating-point format and reduces ex- pensive floating-point multiplications. Häner et al. [25] emphasize the importance of gate scheduling in full-state simulation. They distinguish local and global qubits and propose swapping qubits to reduce the communication overhead between different nodes in a cluster. Pednault et al.[37] adopt a similar idea in the tensor net- work framework. They propose a more systematic gate scheduling algorithm. Unlike these approaches, the goal of SnuQS is to reduce the amount of storage I/O to increase performance and scalability.
\end{comment}

\emph{\textbf{Full-state simulation optimization.}}
Numerous studies have focused on enhancing simulation performance in both homogeneous and heterogeneous systems.
In CPU architectures, the implementation of multithreading alongside AVX vectorization techniques is used to exploit computational resources thoroughly~\cite{qHiPSTER}.
In GPUs, renowned for their massive thread capabilities, maximizing parallelism strategies leads to exceeding performance against homogeneous systems~\cite{QuEST, Aer_sim, cuQuantum}.

% To 更進一步地優化 with increasing 模擬的大小, 部份研究將 QCS 拓展成 多機器或跨節點的版本
% 其中, 這些技法 主要在探討如何 減少溝通時間 with largest bandwidth.
% 要引入這樣的技法往往需要對 給訂的 quantum circuit 做額外的調整.
To further optimize the performance and enlarge the number of qubits, certain studies have extended QCS to encompass multi-rank computer setups.
These techniques primarily concentrate on reducing communication frequency and increasing the transfer bandwidth~\cite{mpiQulacs, cpu_gpu_communication}.
The implementation of these techniques often needs additional adjustments to the order of gate operations in the given quantum circuit.

% Numerous studies have focused on enhancing simulation performance within a single node. Many of these leverage parallel programming techniques, including Single Instruction, Multiple Data (SIMD) instructions, and multithreading, to amplify computation parallelism. Notably, research endeavors comparing CPU and GPU implementations consistently reveal the superior performance of GPU-based simulations.


%Addressing the challenge of simulation performance across multiple nodes, researchers have identified communication links between nodes as a significant bottleneck. Consequently, efforts have been made to alleviate this bottleneck, such as employing a first-in-first-out algorithm to swap global qubits to local qubits~\cite{cache_blocking}. Additionally, innovative approaches like a scheduling method have been proposed to reduce communication overhead further and enhance simulation efficiency, resulting in 45-qubit simulation using 0.5 petabytes~\cite{45qubit}.

% 電路層面是：需要減少ＯＯ
\begin{comment}
\textbf{Quantum Circuit Optimization}
Both the state-of-the-art simulator[25] and SnuQS are based on circuit partitioning techniques. Circuit partitioning is a well- known technique as a variant of graph partitioning. However, the partitioning algorithm’s details heavily depend on the target sys- tem and the simulation method. For example, Pednault et al.[38] allow horizontal circuit partitioning because they use the tensor network contraction algorithm. Häner et al. [25] manually clus- ters a sequence of quantum gates to reduce all-to-all communica- tion. SnuQS uses an automatic circuit partitioning technique based on its qubit permutation and amplitude layout. Moreover, SnuQS prefetches amplitudes to overlap computation and I/O. SnuQS com- bines the circuit partitioning technique with the three-step qubit permutation to guarantee that the I/O operations are grouped in a contiguous block, and the block size is large enough to achieve high I/O bandwidth.
}
\end{comment}

\emph{\textbf{Quantum circuit optimization.}}
%Addressing the challenge of simulation performance across multiple nodes, researchers have identified communication links between nodes as a significant bottleneck. Consequently, efforts have been made to alleviate this bottleneck, such as employing a first-in-first-out algorithm to swap global qubits to local qubits~\cite{cache_blocking}. Additionally, innovative approaches like a scheduling method have been proposed to reduce communication overhead further and enhance simulation efficiency, resulting in 45-qubit simulation using 0.5 petabytes~\cite{45qubit}.
As mentioned earlier, the qubit reordering optimization is developed to minimize the data communication overhead.
In practice, extra fused-swap gates are inserted, and the subsequent target qubit of gates should be adjusted to ensure results accuracy~\cite{cache_blocking, mpiQulacs}.
By using a proper performance tunning technique, the scheduling algorithm enables a 45-qubit simulation using 0.5 petabytes~\cite{45qubit}.

The gate fusion technique is utilized to alleviate the computational load by merging multiple gates into a single generic gate~\cite{45qubit, qHiPSTER, cpu_gpu_communication}.
Although it can reduce the total number of gates, the efficiency of the fused gate is not guaranteed to improve and requires further clarification.
Among numerous fusion techniques, diagonal optimization is a proven technique that can simultaneously reduce the number of gates while keeping high efficiency~\cite{qaoa_arxiv, Lykov_2023}.


%At the circuit level, optimization strategies come into play. Many studies have explored gate fusion ~\cite{qiskit_ae_ana, qHiPSTER} techniques to preprocess the circuit, resulting in an equivalent circuit with fewer gates. This approach contributes to performance improvements in single-node simulations. For scenarios involving multiple nodes, circuit partitioning techniques have been investigated to mitigate inter-node communication, offering a holistic approach to enhancing overall simulation performance.

\begin{comment}
Many state-vector quantum simulators [1, 2, 9, 16, 17, 24, 26, 28–30] have been proposed on supercomputers. 
Qibo [10] uses TensorFlow and custom operators as the backend and supports multi-GPU acceleration. However, Qibo cannot use distributed GPUs across multiple nodes. And Qibo only uses slow CPU-GPU and GPU-to-CPU communication based on PCIe, which costs high communication overhead. 
qHipster [24] performs a number of single- and multi-node optimizations on TACC Stampede supercomputer, including vectorization, multi-threading, cache blocking, as well as overlapping computation with communication. Whereas, it does not support GPU acceleration. 
Our work is implemented on a CPU-GPU heterogeneous cluster. The combination of CPU and GPU allows us to use CPU memory to store many qubits and GPU to accelerate the calculation.

For some state-vector quantum simulators implemented on CPU- GPU heterogeneous clusters, Häner et al. [15] decreased data ex-changes by moving all the gates of the circuits to lower qubits by inserting noiseless swap gates, and employed vectorization and fused multiply-accumulate instructions to exploit the data locality. Our work also exploits data locality on the gate level. Doi et al. [9] proposed a simulator on a heterogeneous high-performance computing system. Then Doi et al. [8] used a scheduling algorithm to quantum supremacy circuits in order to reduce the required communication and simulated a 45-qubit circuit by using 8192 nodes. These works did not reduce the global communication and synchronization overhead for each gate. There is an orthogonality between our scheme and the optimization schemes above. Our work can be attached to the above simulators and provide better performance. In addition, Zhang et al.[30] advocated copying the state to shared memory to reduce the number of times GPU accesses the global memory.

However, their communication scheme is CPU-centric, which cannot avoid a lot of communication between the host and the GPU and can only be simulated on multiple GPUs on a single node. Qulacs [26] uses gate fusion technology to achieve better performance by combining several gates into one. HyQuas [29] combined two approaches [14, 26] to use shared memory and batch matrix-vector multiplication to optimize the communication between GPUs. However, HyQuas failed to utilize the hybrid CPU-GPU memory hierarchy to support large-scale quantum circuits on a limited number of nodes.\textbf{}
\end{comment}
